Collective sleep and activity patterns of college students from wearable devices

To optimize interventions for improving wellness, it is essential to understand habits, which wearable devices can measure with greater precision. Using high temporal resolution biometric data taken from the Oura Gen3 ring, we examine daily and weekly sleep and activity patterns of a cohort of young adults (N=582) in their first semester of college. A high compliance rate is observed for both daily and nightly wear, with slight dips in wear compliance observed shortly after waking up and also in the evening. Most students have a late-night chronotype with a median midpoint of sleep at 5AM, with males and those with mental health impairment having more delayed sleep periods. Social jetlag, or the difference in sleep times between free days and school days, is prevalent in our sample. While sleep periods generally shift earlier on weekdays and later on weekends, sleep duration on both weekdays and weekends is shorter than during prolonged school breaks, suggesting chronic sleep debt when school is in session. Synchronized spikes in activity consistent with class schedules are also observed, suggesting that walking in between classes is a widespread behavior in our sample that substantially contributes to physical activity. Lower active calorie expenditure is associated with weekends and a delayed but longer sleep period the night before, suggesting that for our cohort, active calorie expenditure is affected less by deviations from natural circadian rhythms and more by the timing associated with activities. Our study shows that regular sleep and activity routines may be inferred from consumer wearable devices if high temporal resolution and long data collection periods are available.

==> bin/countcheckboxes-total <==
#!/usr/bin/perl

undef $/;
    $counts=0;
foreach $file (@ARGV) {
    open (FILE, "$file") or die "can't open $file: $!\n";

    $text = <FILE>;
    while ($text =~ m/\\todo{/g) {
	$counts++;
    }
    close FILE;
}
print "$counts";


==> bin/rename <==
#!/usr/bin/perl

$usage = "rename text1 text2 file [files...]

swap text1 for text2 in file names
whenever text1 is found.

swaps only the first instance.

rudimentary first version: use only for static text.
";

$pattern1 = $ARGV[0];
$pattern2 = $ARGV[1];

foreach $filename (@ARGV[2..$#ARGV]) {
    if ($filename =~ m/$pattern1/) {
	($newfilename = $filename) =~ s/$pattern1/$pattern2/g;
	print "renaming $filename as $newfilename...\n";
	`mv "$filename" "$newfilename"`;
    }
}

